Few-shot Personalized Scanpath Prediction

A personalized model for scanpath prediction provides insights into the visual preferences and attention patterns of individual subjects. However, existing methods for training scanpath prediction models are data-intensive and cannot be effectively personalized to new individuals with only a few available examples. In this paper, we propose few-shot personalized scanpath prediction task (FS-PSP) and a novel method to address it, which aims to predict scanpaths for an unseen subject using minimal support data of that subject's scanpath behavior. The key to our method's adaptability is the Subject-Embedding Network (SE-Net), specifically designed to capture unique, individualized representations for each subject's scanpaths. SE-Net generates subject embeddings that effectively distinguish between subjects while minimizing variability among scanpaths from the same individual. The personalized scanpath prediction model is then conditioned on these subject embeddings to produce accurate, personalized results. Experiments on multiple eye-tracking datasets demonstrate that our method excels in FS-PSP settings and does not require any fine-tuning steps at test time. Code is available at: https://github.com/cvlab-stonybrook/few-shot-scanpath

==> tables/adaptation-time.tex <==
\begin{table}[h!]
    \centering
    \renewcommand{\arraystretch}{1} % Adjust row height
    \setlength{\tabcolsep}{1pt} % Adjust column separation    
    \resizebox{1.01\columnwidth}{!}{
    \begin{tabular}{C{1.5cm}C{2.4cm}C{2.4cm}C{2.0cm}}
        \toprule
         &  ChenLSTM-ISP & Gazeformer-ISP & ISP-SENet \\
        \midrule
        Time(s) & 161 & 267 & 3.62 \\
        \bottomrule
    \end{tabular}
    }
    \vskip -0.1in
    \caption{Adaptation time comparison on different methods under 10-shot setting. \label{tab:adaptation-time} }     
\end{table}
\vspace{1mm}

==> tables/distinct.tex <==
\begin{table*}[h!]
    \centering
    \renewcommand{\arraystretch}{1.2} % Adjust row height
    \setlength{\tabcolsep}{3pt} % Adjust column separation    
     
    \begin{tabular}{c|c|ccc|ccc|ccc}
        \multirow{2}{*}{Method} & \multirow{2}{*}{own embedding?} & \multicolumn{3}{c|}{\textbf{OSIE}} & \multicolumn{3}{c|}{\textbf{COCO-FreeView}} & \multicolumn{3}{c}{\textbf{COCO-Search18}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        & & SM $\uparrow$ & MM $\uparrow$ & SED $\downarrow$ & SM $\uparrow$ & MM $\uparrow$ & SED $\downarrow$ & SM $\uparrow$ & MM $\uparrow$ & SED $\downarrow$ \\
        \midrule

        \multirow{2}{*}{ISP(Seen)}
        & $\checkmark$ & 0.386 & 0.814 & 7.003 & - & - & - & 0.468 & 0.815 & 2.475 \\
        & $\times$ & 0.379 & 0.812 & 7.163 & - & - & - & 0.458 & 0.815 & 2.484 \\
        \midrule
        \multirow{2}{*}{Ours(Seen)} 
        & $\checkmark$ & 0.387 & 0.815 & 7.009 & - & - & - & 0.499 & 0.817 & 2.114 \\
        & $\times$ & 0.373 & 0.810 & 7.360 & - & - & - & 0.490 & 0.815 & 2.222 \\
        \midrule
        \multirow{2}{*}{Ours(Unseen)} 
        & $\checkmark$ & 0.376 & 0.802 & 7.286 & - & - & - & 0.482 & 0.815 & 2.359 \\
        & $\times$ & 0.361 & 0.800 & 7.340 & - & - & - & 0.478 & 0.813 & 2.374 \\
        \midrule

    \end{tabular}
    \vskip -0.1in
\caption{Evaluation on the distinction between subject embeddings. \label{tab:distinct}}     
\end{table*}

